Contracts under Moral Hazard and Adverse Selection

In the classical principal-agent problem, a principal must design a contract to incentivize an agent to perform an action on behalf of the principal. We study the classical principal-agent problem in a setting where the agent can be of one of several types (affecting the outcome of actions they might take). This combines the contract theory phenomena of "moral hazard" (incomplete information about actions) with that of "adverse selection" (incomplete information about types). We examine this problem through the computational lens. We show that in this setting it is APX-hard to compute either the profit-maximizing single contract or the profit-maximizing menu of contracts (as opposed to in the absence of types, where one can efficiently compute the optimal contract). We then show that the performance of the best linear contract scales especially well in the number of types: if agent has $n$ available actions and $T$ possible types, the best linear contract achieves an $O(n\log T)$ approximation of the best possible profit. Finally, we apply our framework to prove tight worst-case approximation bounds between a variety of benchmarks of mechanisms for the principal.

==> intro_backup.tex <==
\section{Introduction}
\label{sec:intro}

Consider the classical principal-agent problem, wherein one self-interested economic actor (the ``agent'') is hired to take actions on behalf of another (the ``principal''). The problem arises because the agent has little to no stake in the resulting outcome, so the two enter into a contract designed to encourage the agent to take actions in the interest of the principal. Contract theory distinguishes between two fundamental information asymmetries to consider in the design of this contract. The first is \emph{moral hazard}, which occurs when it may be difficult or costly for the principal to monitor the agent's actions. In this case, the agent may take inappropriate actions, e.g. an insured party may begin to act more recklessly since they are shielded from risk. The second is \emph{adverse selection} (also known as screening), where the agent possesses some private information about their type (e.g. how costly it is for them to perform certain actions) before they decide whether to enter the contract. In this case, the agents that enter contract may be biased, e.g. people with pre-existing conditions would prefer to purchase health insurance.

We study the confluence of these two asymmetries, moral hazard and adverse selection, under the 
computational lens. In particular, we consider a simple hidden-action principal-agent g
model~\cite{grossman1992analysis} but generalized to capture multiple possible agent types. In this 
generalized model, there are $T$ types of agents; an agent has type $t \in [T]$ with probability 
$\frac1T$\footnote{For simplicity, we focus on types having uniform probabilities. All of our negative 
results produce uniform probabilities, and all of our positive results can be made to work for (known) and 
nonuniform probabilities.}. A type $t \in [T]$ agent chooses an action $i \in [n]$, unobserved by the 
principal, at personal and type-independent\footnote{It is possible to reduce type-dependent costs to 
type-independent costs, see \Cref{sec:type-dependent-costs}.} cost $\cost{i}$. This results in a 
distribution over the $m$ outcomes; outcome $j \in [m]$ has a forecasted probability of 
$\TypedForecast{t}{i}{j}$  of occurring and is worth a reward value $\reward{j}$ to the principal. We 
group these  the costs into a cost vector $\costvector{}$; the forecast distributions, a forecast tensor \jonnote{I don't think we should describe this as a tensor; we use tensor typesetting notation, but if it were actually a tensor this would mean that we should be treating this as a specific linear operator where types are in some sort of dual space} $\ForecastTensor$; the rewards, a reward vector $\rewardvector{}$. Together, these four pieces of information characterize a (typed) principal-agent problem $\PrincipalAgentProblem$.
\ggnote{Add an example: Possibly health insurance?}
\ggnote{Remove duplication with Preliminaries.}
\ggnote{Describe a contract.}

\jonnote{I felt like we were jumping a little bit too quickly into ``here is a list of 5 different benchmarks that we prove things about'' so I tried to write a bit of a gentler introduction to how the different benchmarks might arise when thinking about the problem. Not attached to this, happy to revert back (and feel free to edit).}

\subsection{Our Results and Techniques}
\subsubsection*{Contracts without types}

Before we proceed to our results, we give a brief sketch of analogous results for the principal-agent 
problem without types. Many of these results appear in \cite{dutting2019simple}, which was the first to 
study contracts through a computational perspective.

Without types, it is possible to efficiently find the optimal contract for a given principal-agent problem 
-- one way to do so is to, for each action, find the optimal contract that induces the agent to play this 
action (which can be done via solving a linear program). However, the optimal contracts that result from 
this optimization procedure are often complex and unnatural: they can be non-monotone (better outcomes for 
the principal don't necessarily correspond to better payments for the agent), non-budget-balanced (the 
principal may pay more than their value for certain outcomes on those outcomes), and can be very sensitive 
to the parameters of the problem (e.g. the forecast probabilities $\ForecastTensor$). 

Such contracts rarely occur in practice. Instead, people tend to use simpler, more-easily understood 
contracts. One of the simplest classes of contracts is the class of \emph{linear contracts} where principal 
transfers a constant $\alpha$ fraction ($\alpha \in [0, 1]$) of their total reward to the agent. 

\cite{dutting2019simple} also show that when there are $n$ actions the best linear contract achieves an 
$O(n)$-approximation to the best overall contract. In fact, their proof further shows that the revenue of 
the best linear contract is an $O(n)$-approximation to the best revenue achievable in the absence of moral 
hazard, when the principal can directly observe (and contract on) the agent's action (this is 
often referred  to in economics as the ``first-best'' outcome). In this case, the principal will persuade 
the agent to take the action $i$ (by paying them $c_i$ iff they play $i$) which maximizes 
$\E_{j \sim F_{i}}[r_{j}] - c_{i}$. In addition to being the optimal revenue in the absence of moral 
hazard,  this quantity can also be viewed as the maximum possible expected welfare -- we will 
henceforth refer  to it as the ``optimal welfare''.  

\subsubsection*{Contracts with types}

With the introduction of agents of varying types, many aspects of the previous story change.

To begin with, it is no longer necessarily true that the best mechanism for the principal consists of 
presenting the agent with a single contract. As is the case in traditional Bayesian mechanism design (which 
also has hidden types), the principal may wish to present the agent with a \emph{menu} of different 
contracts (each specifying how much the principal would transfer for each outcome). Each agent now 
begins by  choosing their most desirable contract from this menu, then picking the action which 
maximizes their utility as a result of this contract. 

In the previous section, it was possible to efficiently (in polynomial time in the inputs) compute the 
optimal contract. Now it is no longer clear how to efficiently compute the optimal menu for multiple types. 
In fact, it is not even clear how to efficiently compute the optimal \textit{single contract} for multiple 
types -- the same LP approach as before now requires solving exponentially many LPs, one for each 
assignment from types to actions. Our first result shows that this difficulty is 
inherent: we show that computation of both the optimal single contract and optimal menu are \ApxHard{}. 
That is, not only is it NP-hard to compute the optimal single contract (/ optimal menu) exactly, there 
exists a constant $\alpha > 1$ such that getting any $\alpha$-approximation to the optimal revenue 
is \NPHard. 

\jonnote{(add a theorem statement here?)} \ggnote{I think we should just reference them and state the thms in Our Results} \jonnote{(I was imagining this would essentially become the results section; most of the material here is a restatement of material in the current results section anyway)}
The computational hardness of computing these optimal mechanisms make it even more important to 
understand the power of simple classes of contracts. For example, how does the revenue of the 
best linear contract (which we can compute in polynomial-time) compare to that of the best single 
contract or best menu of contracts? One way to get such a bound is to look at the best linear contract 
for each type individually and take the best of these contracts: since each individual linear contract achieves an $O(n)$-approximation to the welfare for the corresponding type, and since there are 
$T$ types, this method will result in an $O(nT)$-approximation to the total welfare (and hence to the best 
single contract or best menu). We show that actually, the revenue of the best linear contract is an 
$O(n\log T)$-approximation to the total welfare and that this is tight.

\jonnote{(add theorem statement)}

We next explore the more-fine grained gaps in power between different options available to the principal. 
For example, how much better is the best single contract than the best linear contract (in the presence of 
types)? What fraction of welfare is the best menu guaranteed to achieve? Specifically, we consider the 
following five benchmarks for the principal, in order from least powerful (linear contracts) to most 
powerful (welfare). 

%\jonnote{(insert list of 5 benchmarks)}

%Table INSERT demonstrates our results concerning the worst-case ratios between our five measures.For almost all the gaps... \jonnote{(finish)}

\jonnote{End new stuff}

%Given such a principal-agent problem, several natural questions come up. Perhaps the first and most natural question is how much revenue or profit a principal can obtain.  We consider five different measures on how much profit can be obtained from such a problem.
\begin{itemize}[noitemsep]
  \item \textbf{Menu of Contracts.} In the most general case, the principal designs a menu of contracts, which assigns to each type a contract $\TypedContractVector{t}$. Each contract specifies a nonnegative\footnote{Without the restriction of agent limited liability, the issue of moral hazard vanishes because the principal can transfer all risk by choosing the contract to be a translation of the reward vector $\rewardvector{}$. This reduces the problem to a standard adverse selection problem i.e. an auction.} transfer $\TypedContract{t}{j} \ge 0$ from principal to agent for each possible outcome $j \in [m]$. Presented with such a menu of contracts, the risk-neutral agent of type $t \in [T]$ chooses a type $t' \in [T]$ to report and an action $i \in [n]$ to take\footnote{Some models allow the agent to opt-out entirely from agreeing to a contract and choosing an action, i.e. individual rationality, but this can be modelled by adding a dummy action that costs zero and always results in a dummy outcome that rewards zero.} (i.e. incentive compatibility) to maximize their expected utility $\left[ \sum_j \TypedForecast{t}{i}{j} \TypedContract{t'}{j} \right] - \cost{i}$ (the expected transfer less their cost). The principal's design goal is to maximize their expected profit, which is expected reward less expected transfer. We denote the optimal expected profit of a menu of contracts as $\OMenu \PrincipalAgentProblem$.
  \item \textbf{Single Contract.} In this restricted design space, the principal may only offer a single contract $\ContractVector$ rather than an entire menu. We denote the optimal expected profit of a single contract as $\OSingle \PrincipalAgentProblem$.
  \item \textbf{Linear Contract.} In this restricted design space, the principal not only offers a single contract, but it must further be linear, i.e. there exists some transfer coefficient $\alpha \in [0, 1]$ that represents what fraction of the principal's reward is transferred to the agent: $\contract{j} = \alpha \reward{j}$. Note there is no reason for a principal to consider menus of linear contracts, since the agent would always select the linear contract with the highest transfer coefficient. We denote the optimal expected profit of a linear contract as $\OLinear \PrincipalAgentProblem$.
  \item \textbf{Welfare.} One upper bound on how much profit a menu of contracts could hope to obtain is the expected welfare, referred to in economics as the ``first-best'' outcome. We denote the expected welfare as $\OWelfare \PrincipalAgentProblem$.
  \item \textbf{Type-Aware Single Contract.} Another upper bound on how much profit a menu of contracts could hope to obtain is the profit sans our adverse selection asymmetry. In this case, the principal knows the type of the agent and can present them a single contract $\TypedContractVector{t}$ without worrying about potential type misreports. We denote the optimal expected profit of a type-aware single contract as $\OTypeAware \PrincipalAgentProblem$.
\end{itemize}


\input{fig/table-ratios.tex}
\ggnote{Add a note just stateful.}
\ggnote{Add informal statement of the theorems}
In this work, we present two sets of results. The first set concerns worst-case ratios between these five 
measures, e.g. what fraction of the total welfare is the optimal menu of contracts guaranteed to extract as 
profit, expressed as a function of the number of types $T$, the number of actions $n$, and the number of 
outcomes $m$? This set of results is summarized in \Cref{tab:ratios}, but we draw the reader's attention to 
two key theorems that power most of the others. In our main theorem upper-bounding worst-case ratios, we 
show that the welfare can be at most $O(n \log T)$ times the profit of the optimal \emph{linear} contract.

\begin{restatable}[APX-Hardness]{theorem}{apxhardness}
\label{thm:apx-hard}
Given an instance of $\InstContract$/ $\InstMenu$, it is \ApxHard to compute the 
optimal contract/menu.  In particular, it is \NPHard to compute a contract $x$  
whose value approximates the optimal revenue by $\alpha \approx 0.64$. 
\end{restatable}

Prior work showed that, in the purely moral hazard situation (i.e. $T = 1$), the welfare could be at most $O(n)$ times the profit of the optimal linear contract (see e.g. proof of Theorem 5.1 from \cite{dutting2019simple}). A \naive{} application of that result would construct the optimal linear contract for each type $t \in [T]$ and pick the best among them. Importantly, linear contracts never result in negative profit since the principal never overpays for any outcome, so this yields a $O(nT)$ bound. Our more careful analysis which considers all types together reduces the $T$ to a $\log T$.

Discuss lower bound construction?

\input{fig/table-computability.tex}

Our second set of results concerns the computability of these five measures, e.g. how much profit could a 
principal with polynomially-bounded computation extract with a menu of contracts? This set of results is 
summarized in \Cref{tab:computability}. In contrast to the purely moral hazard case (i.e. $T = 1$), where 
the best single contract could be computed via a series of polynomially-sized linear programs, 
computing the best single contract is now \ApxHard{}. In other words, there now exists a constant 
$\epsilon > 0$ such that getting a $(1 - \epsilon)$-approximation is \NPHard. We also show that 
menus of contracts are \ApxHard{} to optimize but linear contracts remain polynomial-time.

%\subsection{Story}
%
%Paragraph about contracts and how they're important and moral hazard.
%Paragraph about contracts with types (adverse selection).
%
%We study contracts with multiple types of agent under the computational lens. In particular, we try to understand what can be accomplished by a computationally-limited principal. We explore solution models of varying implementation difficulty, including linear contracts, general single contracts, menus of contracts, full-information contracts, and total welfare.
%
%Cite previous work regarding contracts with types~\cite{???}.
%
%The main question we ask is how much more powerful are menus in the context of multiple types?

    
\subsection{Results}
    \begin{enumerate}
        \item All reasonable negotiations between principal
        and agents can be cast as a menu of contracts. 
        \ggnote{Still to do?}
        \item 
        Each of our 5 classes is a well-studied object in the contracts literature. 
        \item 
        We give strong bounds for all pairs  in the ladder. 
    \end{enumerate}
    
    \input{fig/tikz-roadmap.tex}
    See \Cref{fig:roadmap} for a road map of how we get our lower bounds.
    
    Three main results:
    1) Linear contracts are O(K log T)
    2) The Gap is at least Theta(K log T)
    3) If you have 2 actions and types are in "convex position" then menu can extract full well-fare
    
    
    Computational Results:
    
    There is a way to compute the optimal contract in exponential time
    \begin{enumerate}
    \item For each player $\times$ action compute optimal LP
    
    \item Look at transfer regions (determined by the hyperplanes) and within each region compute the optimal contract. There are only an exponential number of these. 
    \end{enumerate}
    
%\subsection{Technical Section}
%We want to do as well as the best menu. Take the best contract? This gets you a $KT$ fraction. 
%
%Here is a first attempt at proving the bounds and gaps:
%    Budget-Balanced (maybe principal limited liability). 
%    here is a better way ... 

==> notation-table.tex <==
\begin{table}[h]
\begin{tabular}{cc}
  \toprule
  Symbol & Meaning \\ \midrule
  $n$ & number of actions \\
  $m$ & number of outcomes \\
  $T$ & number of types \\
  $i$ & usually action index, esp. subscript \\
  $j$ & usually outcome index, esp. subscript \\
  $t$ & usually type index, esp. parenthetical superscript \\
  $\PrincipalAgentProblem$ & (typed) principal-agent problem \\
  $\ForecastTensor$ & forecast tensor with entries $\TypedForecast{t}{i}{j}$ \\
  $r$ & reward vector with entries $\reward{j}$ \\
  $c$ & cost vector with entries $\cost{i}$ \\
  $R$ & expected reward e.g. $\TypedExpectedReward{t}{i}$ \\
  $\Measure$ & a measure on principal-agent problems (e.g. total welfare, full-information profit) \\
  $\vec{e}_j$ & $j^{th}$ standard basis vector \\
  $\TransferCoefficient$ & transfer coefficient for linear contracts \\
  \bottomrule
\end{tabular}
\caption{\joshnote{Remove this before submission. Cheat sheet for available macros (inspect .tex) and notation. Also, viva booktabs.}}
\end{table}
